Taipan: A Query-free Transfer-based Multiple Sensitive Attribute Inference Attack Solely from Auxiliary Graphs

Graph-structured data underpin a wide spectrum of modern applications, yet their multiple sensitive attributes are not isolated but deeply coupled with graph topology. This coupling facilitates intersectional privacy leakage through attribute inference attacks (AIAs). Existing AIAs predominantly assume adversaries with two capabilities: (I) access to either auxiliary data sampled from the same distribution as the target or partial training records, and (II) the ability to repeatedly query the victim model. In reality, however, these assumptions are often impractical due to stringent data protection regulations, prohibitive query budgets, and heightened detection risks. Moreover, as prior attacks are designed to infer a single sensitive attribute at a time, they fail to simultaneously recover multiple attributes and thus underestimate overall privacy risks arising from cross-attribute dependencies. More critically, they obscure a systemic blind spot: \textbf{auxiliary graphs alone are sufficient to expose multiple sensitive attributes in the target graph.} This threat persists even under distribution shifts, enabling stealthy offline attacks without any model interactions. To investigate this unexplored vulnerability, we introduce \textbf{Taipan, the first query-free framework for multiple sensitive attribute inference attacks on graphs (G-MSAIAs).} Taipan incorporates \emph{Hierarchical Attack Knowledge Routing} to capture intricate inter-attribute correlations, and \emph{Prompt-guided Attack Prototype Refinement} to mitigate distribution shifts between auxiliary and target graphs. Extensive experiments on diverse real-world graph datasets demonstrate that Taipan consistently achieves strong attack performance across same-, similar-, and out-of-distribution settings, and remains effective under partial label coverage or even rigorous privacy guarantees.

==> Related_Work.tex <==
%Tram\`{e}r et al. \cite{Truth_Serum} define targeted and untargeted attribute inference attacks for a single SA. They assume that attackers have access to all features expect for the targeted one, shadow datasets, and the trained model to infer the target attribute of a specific sample. However, their attack settings only target a single SA, and their assumptions are the way too strong.
\section{Related Work}

Due to space limitation, we only discuss the most related research in this section.

\subsection{Attribute Inference Attacks}

\subsubsection{General Neural Network}




\subsubsection{Graph Neural Network}


\subsection{Graph Multi-task Learning}
% Multi-Task Learning (MTL) is a learning paradigm that effectively leverages both task-specific and shared information to address multiple related tasks simultaneously. In contrast to Single-Task Learning (STL), MTL offers a suite of benefits that enhance both the training process and the inference efficiency. MTL’s key advantages encompass streamlined model architecture, performance enhancement, and cross-domain generalizability. From Unleashing the Power of Multi-Task Learning: A Comprehensive Survey Spanning Traditional, Deep, and Pretrained Foundation Model Eras.



\subsection{Graph Prompting}

\subsection{Unsupervised Graph Domain Adaptation}



